Generalized chart constraints for efficient PCFG and TAG parsing

Chart constraints, which specify at which string positions a constituent may begin or end, have been shown to speed up chart parsers for PCFGs. We generalize chart constraints to more expressive grammar formalisms and describe a neural tagger which predicts chart constraints at very high precision. Our constraints accelerate both PCFG and TAG parsing, and combine effectively with other pruning techniques (coarse-to-fine and supertagging) for an overall speedup of two orders of magnitude, while improving accuracy.

==> parsechart.tex <==
\begin{tikzpicture}
% Dark gray background for closed cells
\fill [darkgray] (10,0) -- (11,1) -- (6,6) -- (5,5) -- cycle;
\fill [darkgray] (8,0) -- (9,1) -- (5,5) -- (4,4) -- cycle;
\fill [darkgray] (6,0) -- (7,1) -- (4,4) -- (3,3) -- cycle;
\fill [darkgray] (4,0) -- (5,1) -- (3,3) -- (2,2) -- cycle;

% Light gray background for half-closed cells
\fill [gray] (11,1) -- (12,0) -- (13,1) -- (12,2) -- cycle;
\fill [gray] (7,5) -- (8,4) -- (9,5) -- (8,6) -- cycle;

% Cell borders
\draw (0,0) -- (7,7);
\draw (2,0) -- (8,6);
\draw (4,0) -- (9,5);
\draw (6,0) -- (10,4);
\draw (8,0) -- (11,3);
\draw (10,0) -- (12,2);
\draw (12,0) -- (13,1);

\draw (7,7) -- (14,0);
\draw (6,6) -- (12,0);
\draw (5,5) -- (10,0);
\draw (4,4) -- (8,0);
\draw (3,3) -- (6,0);
\draw (2,2) -- (4,0);
\draw (1,1) -- (2,0);

\draw (0,0) -- (14,0);

% Input tokens
\node at (1,-0.35) {The};
\node at (3,-0.35) {government};
\node at (5,-0.35) {might};
\node at (7,-0.35) {provide};
\node at (9,-0.35) {a};
\node at (11,-0.35) {tax};
\node at (13,-0.35) {credit};

% Cell contents
\node[align=center] at (1,0.35) {DT};
\node[align=center] at (3,0.35) {NN};
\node[align=center] at (5,0.35) {MD};
\node[align=center] at (7,0.35) {VB};
\node[align=center] at (9,0.35) {DT};
\node[align=center] at (11,0.35) {NN};
\node[align=center] at (13,0.35) {NN};

\node[align=center] at (2,1) {NP};
\node[align=center] at (7,6) {S};
\node[align=center] at (9,4) {VP};
\node[align=center] at (10,3) {VP};
\node[align=center] at (11,2) {NP};
\node[align=center] at (12,1) {@NP};

\end{tikzpicture}


==> relwork.tex <==
\section{Related Work} \label{sec:relwork}


\newcite{irtg-ctf-17}: CTF works for PCFGs, but not for more
expressive formalisms.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "irtg-pruning-18"
%%% End:

